Normalising Lustre Preserves Security

The synchronous reactive data flow language LUSTRE is an expressive language, equipped with a suite of tools for modelling, simulating and model-checking a wide variety of safety-critical systems. A critical intermediate step in the formally certified compilation of LUSTRE involves translation to a well-behaved sub-language called "Normalised LUSTRE" (NLUSTRE). Recently, we proposed a simple Denning-style lattice-based secure information flow type system for NLUSTRE, and proved its soundness by establishing that security-typed programs are non-interfering with respect to the co-inductive stream semantics. In this paper, we propose a similar security type system for unrestricted LUSTRE, and show that Bourke et al.'s semantics-preserving normalisation transformations from LUSTRE to NLUSTRE are security-preserving as well. A novelty is the use of refinement security types for node calls. The main result is the preservation of security types by the normalisation transformations. The soundness of our security typing rules is shown by establishing that well-security-typed programs are non-interfering, via a reduction to type-preservation (here), semantics-preservation (Bourke et al.) and our previous result of non-interference for NLUSTRE.

==> LustreStreamSem.tex <==

\subsection{Normalisation Results}\label{app:Normalisation-semantics}

\begin{figure*}
    $$
    \begin{array}{c}
      \mjdg{\semLFby{xs}{ys} = os}
      {\semLFby{(\ccnb{\nullStream}{xs})}{(\ccnb{\nullStream}{ys})} = \ccnb{\nullStream}{os}}  ~~~~
      %
      \mjdg{\semLDFby{y}{xs}{ys} = os}
      {\semLFby{(\ccnb{\stream{x}}{xs})}{(\ccnb{\stream{y}}{ys})} = \ccnb{\stream{x}}{os}}\\
      \\
      \mjdg{\semLDFby{v}{xs}{ys} = os}
      {\semLDFby{v}{(\ccnb{\nullStream}{xs})}{(\ccnb{\nullStream}{ys})} = \ccnb{\nullStream}{os}} ~~~~
      %
      \mjdg{\semLDFby{y}{xs}{ys} = os}
      {\semLDFby{v}{(\ccnb{\stream{x}}{xs})}{(\ccnb{\stream{y}}{ys})} = \ccnb{v}{os}}
    \end{array}
    $$
    \caption{Fby Predicates in \lustre}
    \label{FIG:LusFbyPred}
\end{figure*}

\begin{theorem}[Preservation of semantics. Theorem 2 of \cite{Bourke-jfla2021}]
    \label{THM:JFLA1}
    De-nesting and distribution preserve the semantics of \lustre\ programs. 
    (La passe de d\'{e}simbrication et distributivit\'{e} pr\'{e}serve la s\'{e}mantique des programmes.)
    \[\forall G~ f ~xs~ys, \mstrSemPred{G}{ f(\vv{xs})}{\vv{ys}} \implies \mstrSemPred{\norm{G}}{ f(\vv{xs})}{\vv{ys}}\]
\end{theorem}

\begin{theorem}[Preservation of semantics. Theorem 3 of \cite{Bourke-jfla2021}]
    \label{THM:JFLA2}
    The explicit initialisations of $\ttt{fby}$ preserves the semantics of the programs. 
    (L’explicitation des initialisations pr\'{e}serve la s\'{e}mantique des programmes.)
    \[\forall G~ f ~xs~ys, \mstrSemPred{G}{ f(\vv{xs})}{\vv{ys}} \implies \mstrSemPred{\norm{G}_{fby}}{ f(\vv{xs})}{\vv{ys}}\]
\end{theorem}

==> consolidated_stream_semantics.tex <==

\subsection{Stream Semantics}
\label{SEC:LustreStreamSem}

\begin{figure*}
    $$
    \begin{array}{c}
        \namedJdg{\semConst{c}{bs}{cs}}
        {\mstrSemExpPred{G,\Hst}{bs}{c}{[cs]}}{LScnst} ~~~
        %
        \namedJdg{\Hst(x)={\textcolor{BrickRed}{xs}}}
        {\mstrSemExpPred{G,\Hst}{bs}{x}{[xs]}}{LSvar} \\
        \\
        %
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
            {\liftunop{es}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\unop{e}}{[os]}}{LSunop} \\
        \\
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e_1}{[es_1]}}
            {\mstrSemExpPred{G,\Hst}{bs}{e_2}{[es_2]}}
            {\liftbinop{es_1}{es_2}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\binop{e_1}{e_2}}{[os]}}{LSbinop} \\
        \\
        \namedJdg{\predSet{\forall i ~\mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i}}
            {\hist{x}={\textcolor{BrickRed}{xs}}}
            {\forall i:~\mapwhenk{k}{xs}{\tupstrm{es}_i}{\tupstrm{os}_i}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\when{\vv{e_i}}{x=k}}{
        \flatten{\vv{\tupstrm{os}_i}}}}{LSwhn}\\
        \\
        \namedJdg{\dependSet{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
        {\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}}
        }
        {
           \forall j:~  \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j} 
            ~~~~
            \mapsemIte{es}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}
            }}
        {\mstrSemExpPred{G,\Hst}{bs}{\ite{e}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSite} \\
        \\
       \namedJdg{\dependSet{\predSet{\hist{x}=xs}{
       \forall i: ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}
       }}
            {\forall j: ~
            \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j}
            ~~~~
             \mapsemMerge{xs}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}}
            }
       {\mstrSemExpPred{G,\Hst}{bs}{\lmerge{x}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSmrg} \\
       \\
       \namedJdg{\predSet{\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{e0_i}{\tupstrm{e0s}_i}
      ~~~~ \forall j:~ 
       \mstrSemExpPred{G,\Hst}{bs}{e_j}{\tupstrm{es}_j}}
            { ~\mapsemLFby{(\flatten{\vv{\tupstrm{e0s}_i}})}{
            (\flatten{\vv{\tupstrm{es}_j}})}{\tupstrm{os}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\fby{\vv{e0_i}}{\vv{e_j}}}{\tupstrm{os}}}{LSfby} \\
   \\
        \namedJdg{\forall i \in [1,k] ~ \mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i} ~~~
        [\hist{x_1}, \ldots, \hist{x_n}] = 
        \flatten{\vv{\tupstrm{es}_i}}
        }
        {\mstrEqnPred{G}{\Hst}{bs}{\vv{x_j}=\vv{e_i}}}{LSeqn} \\
  \\
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{LSndef} \\
    \\
           \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{\vv{e_i}}{\tupstrm{xs}}}
            {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{f(\vv{e_i})}{\tupstrm{ys}}}{LSncall}
    \end{array}
    $$
    \caption{Stream semantics of \lustre}
    \label{FIG:LusStrSemNodeEqn}
\end{figure*}
% Name the Rules in a way consistent with the syntax
\begin{figure*}
    $$
    \begin{array}{c}
        \namedJdg{\semConst{c}{bs}{cs}}
        {\mstrSemExpPred{G,\Hst}{bs}{c}{[cs]}}{LScnst} ~~~
        %
        \namedJdg{\Hst(x)={\textcolor{BrickRed}{xs}}}
        {\mstrSemExpPred{G,\Hst}{bs}{x}{[xs]}}{LSvar} \\
        \\
        %
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
            {\liftunop{es}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\unop{e}}{[os]}}{LSunop} \\
        \\
        \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e_1}{[es_1]}}
            {\mstrSemExpPred{G,\Hst}{bs}{e_2}{[es_2]}}
            {\liftbinop{es_1}{es_2}{os} }}
        {\mstrSemExpPred{G,\Hst}{bs}{\binop{e_1}{e_2}}{[os]}}{LSbinop} \\
        \\
        \namedJdg{\predSet{\forall i ~\mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i}}
            {\hist{x}={\textcolor{BrickRed}{xs}}}
            {\forall i:~\mapwhenk{k}{xs}{\tupstrm{es}_i}{\tupstrm{os}_i}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\when{\vv{e_i}}{x=k}}{
        \flatten{\vv{\tupstrm{os}_i}}}}{LSwhn}\\
        \\
        \namedJdg{\dependSet{\predSet{\mstrSemExpPred{G,\Hst}{bs}{e}{[es]}}
        {\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}}
        }
        {
           \forall j:~  \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j} 
            ~~~~
            \mapsemIte{es}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}
            }}
        {\mstrSemExpPred{G,\Hst}{bs}{\ite{e}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSite} \\
        \\
       \namedJdg{\dependSet{\predSet{\hist{x}=xs}{
       \forall i: ~\mstrSemExpPred{G,\Hst}{bs}{et_i}{\tupstrm{ets}_i}
       }}
            {\forall j: ~
            \mstrSemExpPred{G,\Hst}{bs}{ef_j}{\tupstrm{efs}_j}
            ~~~~
             \mapsemMerge{xs}{(\flatten{\vv{\tupstrm{ets}_i}})}{
            (\flatten{\vv{\tupstrm{efs}_j}})}{\tupstrm{os}}}
            }
       {\mstrSemExpPred{G,\Hst}{bs}{\lmerge{x}{\vv{et_i}}{\vv{ef_j}}}{\tupstrm{os}}}{LSmrg} \\
       \\
       \namedJdg{\predSet{\forall i:~ ~\mstrSemExpPred{G,\Hst}{bs}{e0_i}{\tupstrm{e0s}_i}
      ~~~~ \forall j:~ 
       \mstrSemExpPred{G,\Hst}{bs}{e_j}{\tupstrm{es}_j}}
            { ~\mapsemLFby{(\flatten{\vv{\tupstrm{e0s}_i}})}{
            (\flatten{\vv{\tupstrm{es}_j}})}{\tupstrm{os}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{\fby{\vv{e0_i}}{\vv{e_j}}}{\tupstrm{os}}}{LSfby} \\
   \\
        \namedJdg{\forall i \in [1,k] ~ \mstrSemExpPred{G,\Hst}{bs}{e_i}{\tupstrm{es}_i} ~~~
        [\hist{x_1}, \ldots, \hist{x_n}] = 
        \flatten{\vv{\tupstrm{es}_i}}
        }
        {\mstrEqnPred{G}{\Hst}{bs}{\vv{x_j}=\vv{e_i}}}{LSeqn} \\
  \\
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{LSndef} \\
    \\
           \namedJdg{\predSet{\mstrSemExpPred{G,\Hst}{bs}{\vv{e_i}}{\tupstrm{xs}}}
            {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}}
        {\mstrSemExpPred{G,\Hst}{bs}{f(\vv{e_i})}{\tupstrm{ys}}}{LSncall}
    \end{array}
    $$
    \caption{Stream semantics of \lustre}
    \label{FIG:LusStrSemNodeEqn}
\end{figure*}

The semantics of \lustre\ and \nlustre\  programs are \textit{synchronous}:
Each variable and expression defines a data stream which pulses with respect to a \textit{clock}.
A clock is a stream of booleans (CompCert/Coq's $\true$ and $\false$ in Velus).
A flow takes its $n^\tti{th}$ value on the $n^\tti{th}$ clock tick, \textit{i.e.},  some value, written $\stream{v}$, is present at instants when the clock value is \true, and none (written $\nullStream)$ when it is \false.
The \textit{temporal operators} \ttt{when}, \ttt{merge} and \ttt{fby} are used to express the complex clock-changing and clock-dependent behaviours of sampling, interpolation and delay respectively.


%Program behaviours in \lustre\ are completely determined by sequences of clocked occurrences of events.

Formally the stream semantics is defined using predicates over the program graph $G$, a (co-inductive) stream \textit{history} ($\Hst: \tti{Ident} \rightarrow \tti{value}~\tti{Stream}$) that associates value streams to variables, and a clock $bs$ \cite{Lustre2020,PYS-memocode2020,Bourke-jfla2021}.
Semantic operations on (lists of) streams are written in \textcolor{blue}{blue \textsf{sans serif}} typeface.
Streams are written in \textcolor{BrickRed}{red}, with lists of streams usually written in \textbf{\textcolor{BrickRed}{bold face}}.
All these stream operators, defined co-inductively,  enforce the clocking regime, ensuring  the presence of a value when the clock is \ckFont{true}, and absence when \ckFont{false}.

The predicate $\mstrSemExpPred{G,\Hst}{bs}{e}{\tupstrm{es}}$ relates an \textit{expression} $e$ to a \textit{list} of streams, written $\tupstrm{es}$.
A list consisting of only a single stream $\textcolor{BrickRed}{es}$ is explicitly denoted as $\textcolor{BrickRed}{[es]}$.
The semantics of \textit{equations} are expressed using the predicate 
$\mstrEqnPred{G}{\Hst}{bs}{\vv{eqn_i}}$, which requires \textit{consistency} between the assumed and defined stream histories in $\Hst$ for the program variables, as induced by the equations.
Finally, the semantics of \textit{nodes} is given as a stream history transformer predicate
$\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}.$

% Then reference the figure AND 
% explain the rules of the Figure.
Figure \ref{FIG:LusStrSemNodeEqn} presents the stream semantics for \lustre.
While rules for \textit{some} constructs have been variously presented \cite{SNLustre2017,Lustre2020,PYS-memocode2020,Bourke-jfla2021}, our presentation can be considered as a definitive consolidated specification of the operational semantics of \lustre, consistent with the V\'{e}lus compiler encoding \cite{Velus}.

Rule (LScnst) states that a constant $c$ denotes a constant stream of the value $\stream{c}$ pulsed according to given clock $bs$.  
This is effected by the semantic operator \ckFont{const}.
Rule (LSvar) associates a variable $x$ to the stream given by $\Hst(x)$. 
In rule (LSunop), \ckFont{$\hat{\diamond}$} denotes the operation $\diamond$ \textit{lifted} to apply instant-wise to the stream denoted by expression $e$.
Likewise in rule (LSbinop), the  binary operation $\oplus$ is applied paired point-wise to the streams denoted by the two sub-expressions (which should both pulse according to the same clock).
In all these rules, an expression is associated with a \textit{single} stream. 

The rule (LSwhn) describes \textit{sampling} whenever a variable $x$ takes the boolean value $k$, from the flows arising from a list of expressions $\vv{e_i}$,  returning a list of streams of such sampled values.
The predicate $\widehat{\ckFont{when}}$ \textit{maps} the predicate $\ckFont{when}$ to act on the corresponding components of \textit{lists} of streams, \textit{i.e.},  \[ 
\mapwhenk{k}{xs}{[es_1, \ldots, es_k]}{[os_1, \ldots, os_k]} 
~\textrm{abbreviates} ~ 
\bigwedge_{i \in [1,k]}~ \whenk{k}{xs}{es_i}{os_i}.
\]
(Similarly for the predicates
$\widehat{\ckFont{merge}}$, $\widehat{\ckFont{ite}}$, and $\widehat{\ckFont{fby}_L}$.  
The operation $\flatten{\_}$ flattens a list of lists (of possibly different lengths) into a single list. 
Flattening is required since expression $e_i$ may in general denote a \textit{list} of streams \textcolor{BrickRed}{$\tupstrm{es}_i$}.

The expression $\lmerge{x}{\vv{et}_i}{\vv{ef}_j}$ achieves (lists of) streams on a faster clock.
The semantics in rule (LSmrg) assume that for each pair of corresponding component streams from
$\flatten{\tupstrm{ets}_i}$ and
$\flatten{\tupstrm{efs}_j}$, a value is present in the first stream and absent in the second at those instances where $x$ has a true value $\stream{T}$, and complementarily, a value is present in the second stream and absent in the first when $x$ has a false value $\stream{F}$.
Both values must be absent when $x$’s value is absent.
These conditions are enforced by the auxiliary semantic operation \ckFont{merge}. 
In contrast, the conditional expression $\ite{e}{\vv{et}}{\vv{ef}}$
requires that all three argument streams $es$, and the corresponding components from $\flatten{\vv{\tupstrm{ets}_i}}$ and
$\flatten{\vv{\tupstrm{efs}_j}}$ pulse to the same clock.
Again, values are selected from the first or second component streams depending on whether the stream $es$ has the value $\stream{T}$ or $\stream{F}$ at a particular instant.
These conditions are enforced by the auxiliary semantic operation \ckFont{ite}. 
A delay operation is implemented by $\fby{e0}{e}$.
The rule (LSfby) is to be read as follows.
Let each expression $e0_i$ denote a list of streams
$\tupstrm{e0s_i}$, and each expression $e_j$ denote a list of streams $\tupstrm{es_j}$.
The output list of streams consists of streams whose first elements are taken from the each stream in $\flatten{\vv{\tupstrm{e0s}_i}}$ with the rest taken from the corresponding component of $\flatten{\vv{\tupstrm{es}_j}}$.
These are achieved using the semantic operation $\widehat{\ckFont{fby}_L}$.

The rule (LSeqn) for equations checks the consistency between the assumed meanings for the defined variables $x_j$ according to the history $\Hst$ with the corresponding components of the list of streams $\flatten{\vv{\tupstrm{es}_i}}$ to which a tuple of right-hand side expressions evaluates.

The rule (LSndef) presents the meaning given to a node definition $f$ as a stream list transformer. 
If history $\Hst$ assigns lists of streams to the input and output variables for a node a manner such that the semantics of the equations in the node are satisfied, then the semantics $\liftnode{f}$ transforms input stream list $\tupstrm{xs}$ to output stream list $\tupstrm{ys}$.
The operation \ckFont{base-of} finds an appropriate base clock with respect to which a given list of value streams pulse.
The rule (LSncall) uses the stream transformer semantics of $\liftnode{f}$ to the stream list $\tupstrm{xs}$ corresponding to the tuple of arguments $\vv{e_i}$, and returns the stream list $\tupstrm{ys}$.

\paragraph{Clocks and clock-annotated expressions.} \ 
We next present rules for clocks.
Further, we  assume that all (\nlustre) expressions in equations can be clock-annotated, and present the corresponding rules.

\begin{figure*}
$$
   \begin{array}{c}
        \namedJdg{}
        {\mstrSemCkPred{\Hst}{bs}{\ttt{base}}{bs}}{LSbase}  \\ \\
%        
        \namedJdg{
            \dependSet{\predSets{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\true}{bk}}}
            {\hist{x}=\cc{\stream{k}}{xs}}}
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\on{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\on{ck}{x}{k}}{\cc{\true}{bs'}}}{LSonT} \\
        
        
        \namedJdg{
            \dependSet{\predSets{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\false}{bk}}}
            {\hist{x}=\cc{\nullStream}{xs}}}
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\on{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\on{ck}{x}{k}}{\cc{\false}{bs'}}}{LSonA1} 
        \\
               \namedJdg{
            \dependSet{
             \predSet{\mstrSemCkPred{\Hst}{bs}{ck}{\cc{\true}{bk}}}
                {\hist{x}=\cc{\stream{k}}{xs}}
            }
            {\mstrSemCkPred{\htl{\Hst}}{\tl{bs}}{\onF{ck}{x}{k}}{bs'}}}
        {\mstrSemCkPred{\Hst}{bs}{\onF{ck}{x}{k}}{\cc{\false}{bs'}}}{LSonA2} \\ \\


        \namedJdg{\dependSet{\mstrSemExpPred{\Hst}{bs}{e}{[\ccnb{\nullStream}{es}]}}
        {\mstrSemCkPred{\Hst}{bs}{ck}{\ccnb{\false}{cs}}}}
    {\mstrSemExpPred{\Hst}{bs}{e::ck}{[\ccnb{\nullStream}{es}]}}{NSaeA} ~~
    
        \namedJdg{\dependSet{\mstrSemExpPred{\Hst}{bs}{e}{[\ccnb{\stream{v}}{es}]}}
            {\mstrSemCkPred{\Hst}{bs}{ck}{\ccnb{\true}{cs}}}}
        {\mstrSemExpPred{\Hst}{bs}{e::ck}{[\ccnb{\stream{v}}{es}]}}{NSae} 
    \end{array}
$$   
    \caption{Stream semantics of clocks and annotated expressions}
    \label{FIG:StrSemCk}
\end{figure*}

The predicate 
$\mstrSemCkPred{\Hst}{bs}{ck}{bs'}$ in \autoref{FIG:StrSemCk} defines the meaning of a \nlustre\ clock expression $ck$ with respect to a given history $\Hst$ and a clock $bs$ to be the resultant clock $bs'$.
% Note that a clock is a stream of booleans.  
The \ttt{on} construct lets us define 
coarser clocks derived from  a given clock --- whenever a variable $x$ has the desired value $k$ and the given clock is true. 
The rules (LSonT), (LSonA1), and (LSonA2) 
present the three cases: respectively when variable $x$ has the desired value $k$ and clock is true; the clock is false; and  the program variable $x$ has the complementary value and the clock is true.
The auxiliary operations \ckFont{tl} and \ckFont{htl},  give the tail of a stream, and the tails of streams for each variable according to a given history $\Hst$. 
Rules (NSaeA)-(NSae) describe the semantics of  clock-annotated expressions, where the output stream carries a value exactly when the clock is true.

\paragraph{Stream semantics for \nlustre.} \ \ 
The semantic relations for \nlustre\ are either identical to (as in constants, variables, unary and binary operations) or else the (simple) singleton cases of the rules given for \lustre\ (as in \ttt{merge}, \ttt{ite}, \ttt{when}).

The significant differences are in treatment of \ttt{fby}, and the occurrence of \ttt{fby} and node call only in the context of equations.

\begin{figure*}
   $$
    \begin{array}{c}
    \namedJdg{\dependSet{\predSet{\node \in G}
        {\hist{n.\tbf{in}} = \tupstrm{xs}}
        {\baseOf{\tupstrm{xs}} = bs}}
        {\predSet{\resClk{\Hst}{bs}}
        {\hist{n.\tbf{out}} = \tupstrm{ys}}
        {\forall eq \in \vv{eqn}:~ \mstrEqnPred{G}{\Hst}{bs}{eq}}
         }
    }{\mstrCallPred{G}{\liftnode{f}}{\tupstrm{xs}}{\tupstrm{ys}}}{NSndef'} \\
    \\
%
        \namedJdg{\mstrSemExpPred{\Hst}{bs}{e::ck}{\hist{x}}}
        {\mstrEqnPred{G}{\Hst}{bs}{\eqn{x}{e}{ck}}}{NSeqn} 
\\ 
   \namedJdg{\predSet{\mstrSemExpPred{\Hst}{bs}{e::ck}{[vs]}}
            {\semFby{c}{vs}{\hist{x}}}}
        {\mstrEqnPred{G}{\Hst}{bs}{\eqn{x}{\fby{c}{e}}{ck}}}{NSfby'} \\
\\     
    \namedJdg{\predSet{\mstrSemExpPred{\Hst}{bs}{\vv{e}}{\tupstrm{vs}}}
    {\mstrSemCkPred{\Hst}{bs}{ck}{\baseOf{\tupstrm{vs}}}}
    {\mstrCallPred{G}{\liftnode{f}}{\tupstrm{vs}}{\vv{\hist{x_i}}}}}
            {\mstrEqnPred{G}{\Hst}{bs}
        {\eqn{\vv{x}}{f(\vv{e})}{ck}  }}{NSncall'}
   
   \end{array}%  
    $$
    
    \caption{Stream semantics of \nlustre\ nodes and equations}
    \label{FIG:StrSemNodeEqn}
\end{figure*}

The (NSndef') rule only differs from (LSndef) in that 
post-transcription clock alignment, we have an additional requirement of $\Hst$ being in accordance with the base clock $bs$, enforced by \ckFont{respects-clock}.
The (NSdefn) rule for simple equations mentions the clock that annotates the defining expression, checking that it is consistent with the assumed history for the defined variable $x$.
The (NSdelay') rule for \ttt{fby} in an equational context uses the semantic operation \ckFont{fby}, which differs from $\ckFont{fby}_L$ in that it requires its first argument to be a constant rather than a stream.
Finally, the rule rule (NSncall') for node call, now in an equational context, is similar to (LSncall) except that it constrains the clock modulating the equation to be the base clock of the input flows.



==> pred_definitions.tex <==
The definitions of free variables ($fv$) in expressions and equations, and defined variables ($dv$) in equations are given in \autoref{FIG:FVEdef} and \autoref{FIG:FVEQdef}.

\begin{figure}[ht]
\[
\begin{array}{rcl}
    fv(c) &=& \{\}  \\
    fv(x) &=& \{x\}  \\
    fv(\unop{e})&=& fv(e) \\
    fv(\binop{e_1}{e_2})&=& \union{fv(e_1)}{fv(e_2)}\\
    fv(\when{e}{x=k})&=&\union{fv(e)}{\set{x}}\\
    fv(\lmerge{x}{e_1}{e_2}) &=& 
     \union{\set{x}}{fv(e_1)}{fv(e_2)} \\
    fv(\ite{e_1}{e_2}{e_3}) &=& 
    \bigcup_{i=1..3} {fv(e_i)} \\
%    \union{fv(e_1)}{fv(e_2)}{fv(e_3)}\\
    fv(\ttt{base}) &=& \{\ttt{base}\} \\
    fv(\ck{ck}{x=k}) &=& \union{fv(ck)}{\set{x}} \\ \\
    fv(\vv{e})  &=& \bigcup_i {fv(e_i)} \\
\end{array}
\]
    \caption{Free variables for expressions}
    \label{FIG:FVEdef}
\end{figure}

\begin{figure}[ht]
\[
\begin{array}{c}
    fv(\eqn{x}{ce}{ck}) ~=~ \union{fv(ck)}{fv(ce)} \setminus \{x\} \\
    fv(\eqn{x}{\fby{c}{e}}{ck}) ~=~ \union{fv(ck)}{fv(e)} \setminus \{x\} \\
    fv(\eqn{x}{f(\vv{e})}{ck}) ~=~ \union{fv(ck)}{fv(\vv{e})} \setminus \set{\vv{x}} \\ 
 dv(\eqn{x}{ce}{ck}) ~=~  \{x\} \\
    dv(\eqn{x}{\fby{c}{e}}{ck}) ~=~  \{x\} \\
    dv(\eqn{x}{f(\vv{e})}{ck}) ~=~ \set{\vv{x}} 
\end{array}
\]
    \caption{Free and defined variables for equations}
    \label{FIG:FVEQdef}
\end{figure}

\ignore{
\begin{figure*}[ht]
\begin{minipage}{.3\textwidth}
\begin{align*}
    &fv(x)~ = ~ \{x\}  \\
    &fv(c)~ =~ \{\}  \\
    &fv(\unop{e})~ =~ fv(e) \\
    &fv(\binop{e_1}{e_2})~=~ \union{fv(e_1)}{fv(e_2)}\\
    &fv(\when{e}{x=k})~=~\union{fv(e)}{\set{x}}\\
    &fv(\ttt{base})~=~ \{\ttt{base}\} \\
\end{align*}

\end{minipage}%
\begin{minipage}{.7\textwidth}
\begin{align*}
    &fv(\vv{e})  ~=~ \bigcup_i {fv(e_i)} \\
    &fv(\lmerge{x}{e_1}{e_2}) ~ =~ \\
    &\qquad \union{\set{x}}{fv(e_1)}{fv(e_2)} \\
    &fv(\ite{e_1}{e_2}{e_3})~ =~ \\
    &\qquad \union{fv(e_1)}{fv(e_2)}{fv(e_3)}\\
    &fv(\ck{ck}{x=k}) ~=~ \union{fv(ck)}{\set{x}} \\
\end{align*}

\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{align*}
&dv(\eqn{x}{ce}{ck}) ~=~  \{x\} \\
    &dv(\eqn{x}{\fby{c}{e}}{ck}) ~=~  \{x\} \\
    &dv(\eqn{x}{f(\vv{e})}{ck}) ~=~ \set{\vv{x}} \\
\end{align*}
\end{minipage}%
\begin{minipage}{.7\textwidth}
\begin{align*}
    &fv(\eqn{x}{ce}{ck}) ~=~ \union{fv(ck)}{fv(ce)} \setminus \{x\} \\
    &fv(\eqn{x}{\fby{c}{e}}{ck}) ~=~ \union{fv(ck)}{fv(e)} \setminus \{x\} \\
    &fv(\eqn{x}{f(\vv{e})}{ck}) ~=~ \union{fv(ck)}{fv(\vv{e})} \setminus \set{\vv{x}} \\
\end{align*}
\end{minipage}%
    \caption{Definition of $fv$ and $dv$ functions}
    \label{FIG:FVdef}
\end{figure*}
}

The definitions of the auxiliary semantic stream predicates \ckFont{when}, \ckFont{const}, \ckFont{merge}, \ckFont{ite} are given in \autoref{FIG:Def1}. % and \autoref{FIG:Def2}.

\begin{figure*}[ht]
\[
    \begin{array}{c}
        \namedJdg{\semConst{bs'}{c}{cs'}}
        {\semConst{\cc{\true}{bs'}}{c}{\ccnb{\stream{c}}{cs'}}}{DcnstT} ~~~~
        %
        \namedJdg{\semConst{bs'}{c}{cs'}}
            {\semConst{\cc{\false}{bs'}}{c}{\ccnb{\nullStream}{cs'}}}{DcnstF} 
        \\ \\
%     
        \namedJdg{\predSet{\liftunop{es'}{os'}}{\val{v'}= \unop{v}}}
            {\liftunop{\cc{\stream{v}}{es'}}{
                \ccnb{\stream{v'}}{os'}}}{Dunop}  
        ~~~~
        \namedJdg{\liftunop{es'}{os'}}
                {\liftunop{\cc{\nullStream}{es'}}{
                    \ccnb{\nullStream}{os'}}}{DunopA} 
                \\ \\
%     
        \namedJdg{\liftbinop{es_1'}{es_2'}{os'}}
        {\liftbinop{\cc{\nullStream}{es_1'}}{\cc{\nullStream}{es_2'}}{
            \ccnb{\nullStream}{os'}}}{DbinopA} 
%    
            \\ \\
        \namedJdg{
            \predSet{\liftbinop{es_1'}{es_2'}{os'}}{\binop{v_1}{v_2}=\val{v}}}
        {\liftbinop{\cc{\stream{v_1}}{es_1'}}{\cc{\stream{v_2}}{es_2'}}{
            \ccnb{\stream{v}}{os'}}}{Dbinop}
            \\ \\
%
\namedJdg{es = \ccnb{v}{es'}}
    {\tl{es} = es'}{Dtl} 
~~~~
   \namedJdg{\resClk{\Hst}{bs}{vs}}
    {\resClk{\Hst}{\cc{\false}{bs}}{\cc{\nullStream}{vs}}}{DresA} 
    ~~~~
    \\ \\
%
    \namedJdg{\resClk{\Hst}{bs}{vs}}
    {\resClk{\Hst}{\cc{\true}{bs}}{\cc{\stream{v}}{vs}}}{Dres} 
    ~~~~
    \namedJdg{x \in \tti{dom}(\Hst)}
    {\htl{\Hst}(x) =  \tl{\hist{x}}}{Dhtl}
    \\ \\
    \namedJdg{\baseOf{vs}= ~bs}
    {\baseOf{\cc{\val{v}}{vs}} = ~\ccnb{\true}{bs} }{Dbase1}  
    ~~~~
    \namedJdg{\baseOf{vs}= ~bs}
    {\baseOf{\cc{\nullStream}{vs}} = ~\ccnb{\false}{bs} }{Dbase2}     
    \end{array}
\]
    \caption{Definitions of auxiliary predicates-1}
    \label{FIG:Def1}
\end{figure*}

\begin{figure*}
    \[
    \begin{array}{c}
        \namedJdg{\semMerge{xs'}{ts'}{fs'}{os'}}
        {\semMerge{
            \cc{\stream{T}}{xs'}}
            {\cc{\stream{v_t}}{ts'}}
            {\cc{\nullStream}{fs'}}
            {\ccnb{\stream{v_t}}{os'}}}{DmrgT} 
            \\   \\
%
        \namedJdg{\semMerge{xs'}{ts'}{fs'}{os'}}
        {\semMerge{
            \cc{\stream{F}}{xs'}}
            {\cc{\nullStream}{ts'}}
            {\cc{\stream{v_f}}{fs'}}
            {\ccnb{\stream{v_f}}{os'}}}{DmrgF} 
            \\ \\
%
        \namedJdg{\semMerge{xs'}{ts'}{fs'}{os'}}
        {\semMerge{
            \cc{\nullStream}{xs'}}
            {\cc{\nullStream}{ts'}}
            {\cc{\nullStream}{fs'}}
            {\ccnb{\nullStream}{os'}}}{DmrgA} 
            \\ \\
%
        \namedJdg{\semIte{es'}{ts'}{fs'}{os'}}
        {\semIte{
            \cc{\stream{T}}{es'}}
            {\cc{\stream{v_t}}{ts'}}
            {\cc{\stream{v_f}}{fs'}}
            {\ccnb{\stream{v_t}}{os'}}}{DiteT}  
            \\ \\
            \namedJdg{\semIte{es'}{ts'}{fs'}{os'}}
            {\semIte{
                \cc{ \stream{F}}{es'}}
                {\cc{\stream{v_t}}{ts'}}
                {\cc{\stream{v_f}}{fs'}}
                {\ccnb{\stream{v_f}}{os'}}}{DiteF} 
                \\ \\
            \namedJdg{\semIte{es'}{ts'}{fs'}{os'}}
                 {\semIte{  \cc{\nullStream}{es'}}
                    {\cc{\nullStream}{ts'}}
                    {\cc{\nullStream}{fs'}}
            {\ccnb{\nullStream}{os'}}}{DiteA} \\ 
            \\
            \namedJdg{\whenk{k}{xs'}{es'}{os'}}
            {\whenk{k}{\cc{\stream{k}}{xs'}}{\cc{\stream{v}}{es'}}{\ccnb{\stream{v}}{os'}}}{Dwhk}
            \\ \\
                \namedJdg{\semFby{v}{xs}=ys}
            {\semFby{c}{\cc{\stream{v}}{xs}} = \ccnb{\stream{c}}{ys}}{Dfby} 
            ~~
                \namedJdg{\whenk{k}{xs'}{es'}{os'}}
            {\whenk{k}{\cc{\stream{\neg k}}{xs'}}{\cc{\stream{v}}{es'}}{\ccnb{\nullStream}{os'}}}{DwhA1} 
            \\ \\
        %
            \namedJdg{\semFby{c}{xs}=ys}
            {\semFby{c}{\cc{\nullStream}{xs}} = \ccnb{\nullStream}{ys}}{DfbyA} 
            ~~
            \namedJdg{\whenk{k}{xs'}{es'}{os'}}
            {\whenk{k}{\cc{\nullStream}{xs'}}{\cc{\nullStream}{es'}}{\ccnb{\nullStream}{os'}}}{DwhA2} 
         \\ \\
    \end{array}
    \]
    \caption{Definitions of auxiliary predicates-2}
\end{figure*}

All auxiliary stream operators are defined to behave according to the clocking regime.
For example, the rule (DcnstF) ensures the absence of a value when the clock is \ckFont{false}.
Likewise the unary and binary operators lifted to stream operations \ckFont{$\hat{\diamond}$} and \ckFont{$\hat{\oplus}$} operate only when the argument streams have values present, as in (Dunop) and (Dbinop), and mark absence when the argument streams' values are absent, as shown in (DunopA) and (DbinopA).
The rules (Dtl) and (Dhtl) are obvious.

Note that in the rules (DmrgT) and (DmrgF) for \ckFont{merge}, a value is present on one of the two streams being merged and absent on the other.
When a value is absent on the stream corresponding to the boolean variable, values are absent on all streams (DmrgA).
The rules for \ckFont{ite} require all streams to have values present, \textit{i.e.},  (DiteT) and (DiteF), or all absent, \textit{i.e.}, (DiteA).
We have already discussed the \ck{when} operation.
The \ckFont{fby} operation is a bit subtle, and rule (Dfby) may look non-intuitive.  
However, its formulation corresponds exactly to the Velus formalisation,  ensuring that a value from the first argument stream is prepended exactly when a leading value would have been present on the second argument stream. 
The operation \ckFont{base-of} converts a value stream to a clock, \textit{i.e.}, a boolean stream.
The operation \ckFont{respects-clock} is formulated corresponding to the Velus definition.




\ignore{
\begin{figure*}[ht]
\[
    \begin{array}{c}
 \\
        \namedJdg{\whenk{k}{xs'}{es'}{os'}}
    {\whenk{k}{\cc{\stream{k}}{xs'}}{\cc{\stream{v}}{es'}}{\ccnb{\stream{v}}{os'}}}{Dwhnk}
    ~~
%
    \namedJdg{\whenk{k}{xs'}{es'}{os'}}
    {\whenk{k}{\cc{\stream{\neg k}}{xs'}}{\cc{\stream{v}}{es'}}{\ccnb{\nullStream}{os'}}}{DwhnkA1} 
    ~~
%
    \namedJdg{\whenk{k}{xs'}{es'}{os'}}
    {\whenk{k}{\cc{\nullStream}{xs'}}{\cc{\nullStream}{es'}}{\ccnb{\nullStream}{os'}}}{DwhnkA2} 
 \\ \\
    
    \namedJdg{\semFby{v}{xs}=ys}
    {\semFby{c}{\cc{\stream{v}}{xs}} = \ccnb{\stream{c}}{ys}}{Dfby} 
    ~~
    \namedJdg{\semFby{c}{xs}=ys}
    {\semFby{c}{\cc{\nullStream}{xs}} = \ccnb{\nullStream}{ys}}{DfbyA} 
    \\ \\

    

    \namedJdg{\resClk{\Hst}{bs}{vs}}
    {\resClk{\Hst}{\cc{\false}{bs}}{\cc{\nullStream}{vs}}}{DresA} 
~~
    \namedJdg{\baseOf{vs}= ~bs}
    {\baseOf{\cc{\val{v}}{vs}} = ~\ccnb{\true}{bs} }{Dbase1}  
    \\ \\

    \namedJdg{\resClk{\Hst}{bs}{vs}}
    {\resClk{\Hst}{\cc{\true}{bs}}{\cc{\stream{v}}{vs}}}{Dres} 
    ~~

    \namedJdg{\baseOf{vs}= ~bs}
    {\baseOf{\cc{\nullStream}{vs}} = ~\ccnb{\false}{bs} }{Dbase2} 
    \end{array}
\]
    \caption{Definitions of auxiliary predicates: 2}
    \label{FIG:Def2}
\end{figure*}
}

INSERT THIS LATER
\ignore{
\begin{figure*}
    $$
    \begin{array}{c}
      \mjdg{\semLFby{xs}{ys} = os}
      {\semLFby{(\ccnb{\nullStream}{xs})}{(\ccnb{\nullStream}{ys})} = \ccnb{\nullStream}{os}}  ~~~~
      %
      \mjdg{\semLDFby{y}{xs}{ys} = os}
      {\semLFby{(\ccnb{\stream{x}}{xs})}{(\ccnb{\stream{y}}{ys})} = \ccnb{\stream{x}}{os}}\\
      \\
      \mjdg{\semLDFby{v}{xs}{ys} = os}
      {\semLDFby{v}{(\ccnb{\nullStream}{xs})}{(\ccnb{\nullStream}{ys})} = \ccnb{\nullStream}{os}} ~~~~
      %
      \mjdg{\semLDFby{y}{xs}{ys} = os}
      {\semLDFby{v}{(\ccnb{\stream{x}}{xs})}{(\ccnb{\stream{y}}{ys})} = \ccnb{v}{os}}
    \end{array}
    $$
    \caption{\ckFont{fby} semantic predicates}
    \label{FIG:LusFbyPred}
\end{figure*}
}

==> related_work.tex <==
\section{Related Work}
\label{SEC:related}
\noindent{\bf Security type systems:} 
Denning's seminal paper \cite{Denning:1976} proposed complete lattices as the appropriate structure for information flow analyses. 
The subsequent paper \cite{Denning:1977} presented static analysis frameworks for certifying secure information flow. 
A gamut of secure flow analyses were based on these foundations.

Only much later did Volpano \textit{et al.} \cite{Volpano96} provide a security type system with a semantic soundness result by showing that security-typed programs exhibit non-interference \cite{GoguenM82a}.
Type systems remain a powerful way of analysing program behaviour, particularly secure information flow.
%Types or typed annotations that specify rules regarding the usage of typed variables offer powerful and general ways by which program behaviors can be analysed, {\em vis-\`a-vis} IFC.  
For instance, the {\sc Jif} compiler \cite{jif} for the {\sc JFlow} language \cite{myers_jflow_1999} (based on Java) not only checks for IFC leaks but also deals with {\em declassification}, using the {\em Decentralised model} of data ownership \cite{MyersLiskov1997}. 
Matos \textit{et al} proposed a \textit{synchronous reactive} extension of Volpano's imperative framework.  
Their language is at a lower level than \lustre, and has explicit synchronization primitives for broadcast signals, suspension, preemption and scheduling of concurrent threads.
While they employ the notion of \textit{reactive bisimulation} to deal with concurrency, the techniques employed closely follow Volpano's formulation of the type system (which use \textit{var} and \textit{cmd} types) and a reduction semantics (necessitating a subject reduction theorem).
In contrast, we are able to leverage the declarative elegance and simplicity of \lustre\ to present a far simpler type system and its soundness proof in terms of \lustre's co-inductive stream semantics. \\[1ex]
%
\noindent{\bf Semantics and logics:}
Non-interference \cite{GoguenM82a} is considered a standard semantic notion for security although other notions of semantic correctness have been proposed, \textit{e.g.}, \cite{Boudol08}.
Non-interference is a typical \textit{hyperproperty} \cite{Clarkson2010}, \textit{i.e.}, a set of set of program traces.  
Clarkson \textit{et al} \cite{Rabe2014} have presented temporal logics {\em HyperLTL, HyperCTL$^{*}$}, for verification of hyperproperties. \\[1ex]
%
\noindent{\bf Beyond type systems:}
Zanotti \cite{Zanotti2002} proposed an abstract interpretation framework similar to the earlier work from Volpano \textit{et al}, but strictly more general in its applicability.
Hunt and Sands \cite{HuntSands2006} extended type-based IFC checking with flow-sensitivity.
In {\sc Paragon}, a Java-based language proposed by Broberg \textit{et al.} \cite{Broberg2013}, one can additionally handle the runtime tracking of typestate.
However, in general, type-based techniques can exhibit imprecision as they lack flow and context sensitivity and do not systematically handle unstructured control flow and exceptions in programs.
Hammer and Snelting \cite{hammer_flow-sensitive_2009} proposed the usage of program dependence graphs (PDGs) to offer a flow-, context- and object-sensitive analysis to detect IFC leaks. 
Livshits \textit{et al} \cite{Livshits2009} use data propagation graphs to automatically infer explicit information flow leaks. \\[1ex]
%
\noindent{\bf Runtime techniques:} 
Dynamic analyses provide greater precision, particularly in systems which rely on dynamic typing, when static dependency graph or type-based approaches are not adequate.  
Shroff \textit{et al} \cite{Shroff2007} have proposed dynamic tracking of dependencies to analyse noninterference.  
Austin and Flanagan \cite{AustinFlanagan2009,AustinFlanagan2010} have proposed dynamic checks to efficiently detect implicit flows based on the {\em no-sensitive-upgrade} semantics and the {\em permissive-upgrade} semantics.  
Their subsequent work \cite{AustinFlanagan2017} addressed limitations in the semantics due to which executions where implicit flows cannot be tracked are prematurely terminated. \\[1ex]
%
\noindent{\bf IFC analyses in hardware and systems:}
%
We refer to but do not further discuss here work addressing IFC analyses in hardware systems, \textit{e.g.} \cite{TiwariISCA2011,TiwariASPLOS2014,zhang_hardware_2015,ferraiuolo2018hyperflow}, 
in programming languages \cite{sabelfeld2003language,Pottier2003-FlowCaml,liu2017fabric,roy2009laminar}, in operating systems,   \cite{Krohn2007-aa,zeldovich2006-osdi,cheng2012aeolus,efstathopoulos2005asbestos,roy2009laminar}, and in databases \cite{schultz2013ifdb}.
In the context of embedded systems, it will be interesting to see how our higher-level \lustre-based approach compares with  lower-level secure hardware description languages such as SecVerilog \cite{zhang_hardware_2015} and ChiselFlow \cite{ferraiuolo2018hyperflow} in which fine-grained security policies can be expressed.

% \noindent{\bf Hardware analysis:}
% Tiwari \textit{et al.} \cite{TiwariISCA2011} investigate dynamic IFC tracking at the level of logic gates, but could suffer from  overheads in area or power or issues in scaling the technique to large designs. 
% In subsequent work \cite{TiwariASPLOS2014} adds further logic for tracking information flows. 
% Zhang et al. \cite{zhang_hardware_2015} propose a HDL, SecVerilog, which makes it possible to statically analyse control of timing channels of processor designs. 
% \lustre\ has an added advantage over many HDLs that it comes with clean formal semantics, which enables correct-by-construction compilation of systems.

